Physics-Informed Representation Alignment for Sparse Radio-Map Reconstruction

Radio map reconstruction is essential for enabling advanced applications, yet challenges such as complex signal propagation and sparse observational data hinder accurate reconstruction in practical scenarios. Existing methods often fail to align physical constraints with data-driven features, particularly under sparse measurement conditions. To address these issues, we propose **Phy**sics-Aligned **R**adio **M**ap **D**iffusion **M**odel (**PhyRMDM**), a novel framework that establishes cross-domain representation alignment between physical principles and neural network features through dual learning pathways. The proposed model integrates **Physics-Informed Neural Networks (PINNs)** with a **representation alignment mechanism** that explicitly enforces consistency between Helmholtz equation constraints and environmental propagation patterns. Experimental results demonstrate significant improvements over state-of-the-art methods, achieving **NMSE of 0.0031** under *Static Radio Map (SRM)* conditions, and **NMSE of 0.0047** with **Dynamic Radio Map (DRM)** scenarios. The proposed representation alignment paradigm provides **37.2%** accuracy enhancement in ultra-sparse cases (**1%** sampling rate), confirming its effectiveness in bridging physics-based modeling and deep learning for radio map reconstruction.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sec/proof.tex <==
\section{Proofs}

\section*{Appendix: Derivation of the Path Loss Model}
\label{path loss}
\subsection*{Theorem}
Let $\psi(\mathbf{r})$ represent the time-harmonic solution of the Helmholtz equation in $D$-dimensional free space. The path-loss model in dB at position $\mathbf{r} = (a, b)$, considering $N_t$ transmitters at positions $\mathbf{r}_k = (a_k, b_k)$, is given by:
\[
P(a, b) = \sum_{k=1}^{N_t} \Big(\alpha_k - 10 \theta_k \log_{10} \big(\sqrt{(a_k - a)^2 + (b_k - b)^2}\big) \Big),
\]
where:
\begin{itemize}
    \item $\alpha_k$ is the transmitted power (in dB) at a reference distance,
    \item $\theta_k$ is the path-loss exponent for transmitter $k$.
\end{itemize}

\subsection*{Proof}
\begin{enumerate}
    \item \textbf{Helmholtz Equation}  
    The wave equation for time-harmonic waves in free space is given by:
    \[
    \nabla^2 \psi(\mathbf{r}) + k^2 \psi(\mathbf{r}) = 0,
    \]
    where $\psi(\mathbf{r})$ is the scalar field, and $k = \frac{2\pi}{\lambda}$ is the wavenumber with $\lambda$ being the wavelength.

    \item \textbf{Solution in Free Space}  
    For a point source located at $\mathbf{r}_k$ in $D$-dimensional free space, the general outgoing solution is:
    \[
    \psi_k(\mathbf{r}) = \frac{A_k}{\|\mathbf{r} - \mathbf{r}_k\|^{(D-1)/2}} e^{i k \|\mathbf{r} - \mathbf{r}_k\|},
    \]
    where:
    \begin{itemize}
        \item $\|\mathbf{r} - \mathbf{r}_k\|$ is the radial distance from the $k$-th transmitter,
        \item $D = 3$ for spherical waves,
        \item $D = 2$ for cylindrical waves.
    \end{itemize}

    \item \textbf{Amplitude Decay}  
    The amplitude of the wave decays as:
    \[
    |\psi_k(\mathbf{r})| \sim \frac{1}{\|\mathbf{r} - \mathbf{r}_k\|^{(D-1)/2}}.
    \]
    The \textbf{power}, being proportional to the square of the amplitude, is:
    \[
    P_{\text{linear}, k}(\mathbf{r}) \propto \frac{1}{\|\mathbf{r} - \mathbf{r}_k\|^{D-1}}.
    \]

    \item \textbf{Power in dB Scale}  
    Converting the linear-scale power to dB scale:
    \[
    P_{\text{dB}, k}(\mathbf{r}) = -10 (D-1) \log_{10}(\|\mathbf{r} - \mathbf{r}_k\|) + C_k,
    \]
    where $C_k = 10 \log_{10}(P_{0,k})$ is a constant accounting for the reference power $P_{0,k}$ at a reference distance $\|\mathbf{r}_0\|$ for the $k$-th transmitter.

    \item \textbf{General Path-Loss Exponent}  
    In real environments, the decay rate is generalized by introducing a path-loss exponent $\theta_k$, which accounts for effects like reflection, diffraction, and scattering:
    \[
    P_{\text{dB}, k}(\mathbf{r}) = -10 \theta_k \log_{10}(\|\mathbf{r} - \mathbf{r}_k\|) + C_k.
    \]
    Here, $\theta_k$ may differ from $D-1$ due to environmental factors.

    \item \textbf{Multi-Transmitter Model}  
    For $N_t$ transmitters located at positions $\mathbf{r}_k = (a_k, b_k)$, the total received power at $\mathbf{r} = (a, b)$ is modeled as the sum of contributions from all transmitters:
    \[
    P(a, b) = \sum_{k=1}^{N_t} P_k(a, b),
    \]
    where $P_k(a, b)$ is the power contribution from the $k$-th transmitter:
    \[
    P_k(a, b) = \alpha_k - 10 \theta_k \log_{10} \big(\|\mathbf{r} - \mathbf{r}_k\|\big).
    \]
    Here, $\alpha_k = C_k$ represents the reference power in dB, and $\|\mathbf{r} - \mathbf{r}_k\| = \sqrt{(a_k - a)^2 + (b_k - b)^2}$ is the Euclidean distance in 2D space. For 3D space, the distance would include a $z$-component:
    \[
    \|\mathbf{r} - \mathbf{r}_k\| = \sqrt{(a_k - a)^2 + (b_k - b)^2 + (z_k - z)^2}.
    \]

    Substituting the 2D Euclidean distance, the total power becomes:
    \[
    P(a, b) = \sum_{k=1}^{N_t} \Big(\alpha_k - 10 \theta_k \log_{10} \big(\sqrt{(a_k - a)^2 + (b_k - b)^2}\big)\Big).
    \]
\end{enumerate}

\subsection*{Parameter Optimization}
To fit the model to observed data, let $\{x(j), c(j)\}_{j=1}^{K_i}$ be $K_i$ observations, where $x(j)$ is the power at location $c(j)$. The parameters $\{\alpha_k, \theta_k\}$ are optimized by minimizing the squared error:
\[
\min_{\{\alpha_k, \theta_k\}} \sum_{j=1}^{K_i} \Big( x(j) - P(c(j)) \Big)^2,
\]
where $P(c(j))$ is the modeled power at location $c(j)$. Additional constraints or regularization terms may be included to improve the robustness of the optimization, such as:
\[
\min_{\{\alpha_k, \theta_k\}} \left( \sum_{j=1}^{K_i} \Big( x(j) - P(c(j)) \Big)^2 + \lambda \sum_{k=1}^{N_t} (\theta_k - \bar{\theta})^2 \right),
\]
where $\lambda$ is a regularization parameter and $\bar{\theta}$ is a prior estimate of the path-loss exponent.

\subsection*{Conclusion}
The path-loss model is derived as:
\[
P(a, b) = \sum_{k=1}^{N_t} \Big(\alpha_k - 10 \theta_k \log_{10} \big(\sqrt{(a_k - a)^2 + (b_k - b)^2}\big) \Big),
\]
where $\alpha_k$ and $\theta_k$ are fitted to observed data. The model reflects the physical principles of wave propagation generalized for real-world environments, with the following assumptions and limitations:
\begin{itemize}
    \item The model assumes no interference between transmitters.
    \item Environmental effects like shadowing and multipath are not explicitly included.
    \item The dimensionality $D$ is assumed to be 2; for 3D scenarios, the distance formula must be adjusted.
\end{itemize}


In \LaTeX{} proofs should be typeset using the \texttt{\textbackslash{proof}} environment.

\begin{proof}
    This paragraph is an example of how a proof looks like using the \texttt{\textbackslash{proof}} environment.
\end{proof}


\section{Algorithms and Listings}

Algorithms and listings are a special kind of figures. Like all illustrations, they should appear floated to the top (preferably) or bottom of the page. However, their caption should appear in the header, left-justified and enclosed between horizontal lines, as shown in Algorithm~\ref{alg:algorithm}. The algorithm body should be terminated with another horizontal line. It is up to the authors to decide whether to show line numbers or not, how to format comments, etc.

In \LaTeX{} algorithms may be typeset using the {\tt algorithm} and {\tt algorithmic} packages, but you can also use one of the many other packages for the task.

\begin{algorithm}[tb]
    \caption{Example algorithm}
    \label{alg:algorithm}
    \textbf{Input}: Your algorithm's input\\
    \textbf{Parameter}: Optional list of parameters\\
    \textbf{Output}: Your algorithm's output
    \begin{algorithmic}[1] %[1] enables line numbers
        \STATE Let $t=0$.
        \WHILE{condition}
        \STATE Do some action.
        \IF {conditional}
        \STATE Perform task A.
        \ELSE
        \STATE Perform task B.
        \ENDIF
        \ENDWHILE
        \STATE \textbf{return} solution
    \end{algorithmic}
\end{algorithm}

\section{\LaTeX{} and Word Style Files}\label{stylefiles}

The \LaTeX{} and Word style files are available on the IJCAI--25
website, \url{https://2025.ijcai.org/}.
These style files implement the formatting instructions in this
document.

The \LaTeX{} files are {\tt ijcai25.sty} and {\tt ijcai25.tex}, and
the Bib\TeX{} files are {\tt named.bst} and {\tt ijcai25.bib}. The
\LaTeX{} style file is for version 2e of \LaTeX{}, and the Bib\TeX{}
style file is for version 0.99c of Bib\TeX{} ({\em not} version
0.98i). .

The Microsoft Word style file consists of a single file, {\tt
        ijcai25.docx}. 
%This template differs from the one used for IJCAI--23.

These Microsoft Word and \LaTeX{} files contain the source of the
present document and may serve as a formatting sample.

Further information on using these styles for the preparation of
papers for IJCAI--25 can be obtained by contacting {\tt
        proceedings@ijcai.org}.

\appendix

\section*{Ethical Statement}

There are no ethical issues.

\section*{Acknowledgments}

The preparation of these instructions and the \LaTeX{} and Bib\TeX{}
files that implement them was supported by Schlumberger Palo Alto
Research, AT\&T Bell Laboratories, and Morgan Kaufmann Publishers.
Preparation of the Microsoft Word file was supported by IJCAI.  An
early version of this document was created by Shirley Jowell and Peter
F. Patel-Schneider.  It was subsequently modified by Jennifer
Ballentine, Thomas Dean, Bernhard Nebel, Daniel Pagenstecher,
Kurt Steinkraus, Toby Walsh, Carles Sierra, Marc Pujol-Gonzalez,
Francisco Cruz-Mencia and Edith Elkind.

